Learning Neural Networks with Sparse Activations

A core component present in many successful neural network architectures, is an MLP block of two fully connected layers with a non-linear activation in between. An intriguing phenomenon observed empirically, including in transformer architectures, is that, after training, the activations in the hidden layer of this MLP block tend to be extremely sparse on any given input. Unlike traditional forms of sparsity, where there are neurons/weights which can be deleted from the network, this form of {\em dynamic} activation sparsity appears to be harder to exploit to get more efficient networks. Motivated by this we initiate a formal study of PAC learnability of MLP layers that exhibit activation sparsity. We present a variety of results showing that such classes of functions do lead to provable computational and statistical advantages over their non-sparse counterparts. Our hope is that a better theoretical understanding of {\em sparsely activated} networks would lead to methods that can exploit activation sparsity in practice.

==> rademacher-attempts.tex <==
\section{Attempts for improved Rademacher bound}
\paragraph{Understanding extreme cases of \texorpdfstring{\Cref{thm:rademacher-1-sparse}}{Theorem~\ref{thm:rademacher-1-sparse}}.}

Let's analyze \Cref{eq:1} in the case of two extreme datasets $S_1$ and $S_2$, where
\begin{itemize}
\item $S_1$ consists of $m$ orthogonal vectors, and
\item $S_2$ consists of the same vector $m$ times, that is, $x_1 = \ldots = x_m = x_*$.
\end{itemize}

\noindent In the case of $S_1$, we have that $\sqrt{\sum_j T_j^2} \le B' \sqrt{m}$. Hence, we get a final bound of $\frac{BB'}{\sqrt{m}}$.\\

\noindent In the case of $S_2$, we can assume wlog that only $T_1$ is non-zero and the other $T_j$'s are zero. In this case, we have that
\[
\E_{\sigma} \max_f T_1 ~=~ \E_{\sigma} \max_f \sum_{i=1}^m \sigma_i g_1(x_*) = B' \E_{\sigma} \left | \sum_{i=1}^m \sigma_i \right | \le B' \sqrt{m}
\]
Thus, again we get a final bound of $\frac{BB'}{\sqrt{m}}$.\\

The thing to observe is that we get the desired bound of $\frac{BB'}{\sqrt{m}}$ in both cases, due to fundamentally different reasons. Can we interpolate between these two reasons for arbitrary datasets?

Let's consider the following dataset $S$ consisting of $m$ vectors such that inner product of any two distinct vectors is $1 - \eps$. For example, this is possible in $d = m+1$ dimensions, where $x_i = (\sqrt{1 - \eps}, 0, ... , 0, \sqrt{\eps}, 0, \ldots)$ with $\sqrt{\eps}$ in the $(i+1)$-th coordinate (although, could be possible using fewer dimensions).


\paragraph{[Buggy - doesn't work] Possible idea to get $1/\sqrt{m}$ dependence while being independent of $s$}

Let us go back to Step~\eqref{eq:1} in the above proof. The key quantity to bound is the following:
\begin{align}
     \mathbb{E}_\sigma \max_f  \sqrt{\sum_j T^2_j}
\end{align}
We know from the Rademacher complexity of a single ReLU unit that for any fixed $j$,
\begin{align}
    Pr_\sigma \left[\max_{w} T_j \le O(B'\sqrt{dm\log(s)})\right] >= 1 - 1/10s .\label{eq:2}
\end{align}
(verify this statement)

Given a function $f \in H_1$, and a train set $S = \{x_i\}_{i=1}^m$, let $m_j$ denote the number of examples which activate neuron $j$. Using this and \ref{eq:2}, we want to claim that

Define random variable $Y_j = \max_w T_j$. Then, 
$$E[Y_j^2] \leq E[\max_w (\sum_{i=1}^m \sigma_i g_j(x_i))^2].$$
\begin{align}
     \mathbb{E}_\sigma \max_f  \sqrt{\sum_j T^2_j} &\le  \sqrt{\mathbb{E}_\sigma \max_f \sum_j T^2_j} \le \sqrt{\sum_j m_jB'^2d\log(s)} \\
     &\le \sqrt{mB'^2d\log(s)},
\end{align}
which is the bound with ideal dependence on $s$ and $m$.

\subsection{Improved Rademacher complexity bound}

In order to improve the Rademacher complexity bound, we use the following proposition.
\begin{proposition}\label{prop:margin-halfspaces}
For all $x_1, \ldots, x_m \in \B^d(1)$, there exist at most $m^{1/\gamma^2}$ distinct labelings $y_1, \ldots, y_m \in \{-1,1\}^m$ such that there exists $w \in \B^d(1)$ satisfying $y_i \ang{w, x_i} \ge \gamma$ for all $i \in [m]$.
\end{proposition}

We use a slightly stronger version of the above proposition.
\begin{proposition}\label{prop:margin-halfspaces-v2}
For all $x_1, \ldots, x_m \in \B^d(1)$, there exist at most $m^{1/\gamma^2}$ distinct labelings $y_1, \ldots, y_m \in \{-1,1\}^m$ such that there exists $w \in \B^d(1)$ satisfying:
\begin{itemize}
\item $y_i \ang{w, x_i} > 0$ for all $i \in [m]$, that is, all points are correctly classified, and
\item $\frac{1}{|S_+|} \sum_{i \in S_+} \ang{w, x_i} \ge 2\gamma$ for $S_+ = \{i : y_i = +1\}$, points on positive side are classified with an average margin of $2\gamma$.\pritish{Wait, how did we go from worst-case margin to average margin?}
\end{itemize}
\end{proposition}

\begin{theorem}\label{thm:rademacher-1-sparse-v2}
It holds that
\begin{align}
\mathcal{R}_{H_1(B, B')}(S) &~:=~ \mathbb{E}_\sigma \sq{\max_{f \in H_1} \frac{1}{m} \sum_{i=1}^m \sigma_i \sum_{j=1}^s u_j \relu(\ang{W_j, x_i})} ~\leq~ \frac{BB'}{m^{\frac 1 3}}.
\end{align}
\end{theorem}
\begin{proof}
As before, for any $x_i$, define $g_j(x_i) = \relu(W_j \cdot x_i)$ and define $\vec{g}(x_i)$ to be the $s$-dimensional vector. Let $S_j := \{i \in [m] \,:\, \ang{W_j, x_i} > 0\}$. By assumption of $1$-sparsity, we know that $S_j$'s are pairwise disjoint. As before, we have\pritish{I think the below inequality holds with equality?}
\begin{align*}
\mathcal{R}_{H_1}(S) &\leq B \mathbb{E}_\sigma \left[ \max_f \left\|\frac 1 m \sum_{i=1}^m \sigma_i \vec{g}(x_i)\right\| \right].
\end{align*}
We have
\begin{align*}
\left \|\frac1m \sum_{i=1}^m \sigma_i \vec{g}(x_i) \right \|  = \frac1m \prn{\sum_{j=1}^s \prn{\sum_{i \in S_j} \sigma_i \cdot \relu(\ang{W_j, x_i})}^2}^{1/2}
\end{align*}
(Unfinished)
\end{proof}


\subsection{Possible approach to get \texorpdfstring{$\sqrt{d/m}$}{sqrt(d/m)} Rademacher}
Let us first look at the case $k=1, d=2$. In this case, if the inputs $x_i$ all lie within the unit circle, each neuron is choosing a different circular segment of the unit circle to decide which inputs are active. Sparsity requires that the different circular segments are all non-overlapping.

We can assume that each circular segment corresponds to an angle $\le \pi/2$ at the center of the circle. (if this is not true, there can't be too many segments with angles $> \pi/2$ and each such segment's individual contribution to $\sum_j T_j^2$ should be easy to bound). This will allow us to also assume that for every point $x_i$ within a segment, the corresponding dot product $\ang{w_j, x_i} = 1$. This is approximately true and doesn't affect the bounds much when $d=2$. (For larger $d$, the dot products can be as small as $1/\sqrt{d}$ and this probably helps us avoid a dependence on $d$ showing up in the final bound.)

Now, the problem simplifies. Each $T_j$ becomes simply the sum of the signs $\sigma$ which activate neuron $j$. We first arrange the points $x_1, x_2, \ldots, x_m$ in a line so that each $T_j$ represents a contiguous subset (this is obvious if points lie exactly on the unit circle. even if some points lie inside should be able to linearize somehow?). Consequently, the task of the adversary is to find a partitioning of the $m$ signs organized in a line into $s+1$ subsets (an additional subset to capture no neuron being active) so as to maximize $\sum_j T_j^2$.

Due to concentration, with probability $\ge 1-1/m^{100}$, we have that simultaneously for all $i_1 < i_2$,
$$\left|\sum_{i=i_1}^{i_2} \sigma_i\right| \le c\sqrt{(i_2-i_1)\log(m)},$$
for a large enough constant $c$.
Therefore,
\begin{align*}
    \sum_j T_j^2 \le c^2\log(m) m,
\end{align*}
which is the desired bound.
Its important to note that the above bound holds no matter the partitioning chosen by the adversary. Hence we aren't union bounding over all possible partitions (which will be $O(m^s)$ and too many to union bound over).

For larger $d$, we need to union bound over $O(m^d)$ possible spherical caps and consequently it should be possible to generalize the above argument to get
\begin{align*}
    \sum_j T_j^2 \le c^2d\log(m) m.
\end{align*}

This ignores the fact that dot products can decay very rapidly as $d$ increases and that decay will likely cancel out the additional $d$ factor. (If the points were distributed in close clusters so that the decay of dot products is avoinded, this would in turn drastically reduce the number of distinct spherical caps possible from $O(m^d)$ to a much smaller number possibly removing the $d$ factor in the process again.

==> s5-ub-general.tex <==
\section{Learning over Arbitrary Distributions : Upper Bounds}\label{sec:ub-general}
In this section we study the learnability of sparsely activated one layer ReLU networks under arbitrary distributions. We will first consider the class $\cH_{n,s,1}$, i.e., the class of networks where the activation sparsity is $k=1$. In Appendix~\ref{sec:ub-general-k} we extend the results from this section to the more general setting of $\cH_{n,s,k}$. For the results of this section we assume that every function of the form $h(x) = \sum_{i=1}^s u_i \sigma(\ang{w_i,x} - b_i)$ has the following bound on the weights: $\|u\| \max_i (\|w_i\| + |b_i|) \leq B$.
The main result of this section is stated below.
\begin{theorem}
\label{thm:ub-general-1}
$\cH_{n,s,1}$ is $(\eps,\delta)$-PAC learnable with sample complexity $m = \tilde{O}\left(\frac{n^2 B^2 s \log(\frac 1 \delta)}{\eps^2} \right)$ and running time $\tilde{O}\left(s \cdot m \cdot 2^{\tilde{O}(n)}\right)$.
\end{theorem}

Note that in the above theorem, the sample complexity has a polynomial dependence on both $n$ (input dimensionality) and $s$ (number of hidden units). The key computational advantage we achieve via the promise of sparsity is that the runtime dependence is linear in $s$ and only has an exponential dependence on the input dimensionality $n$. In contrast, it is not known how to learn general depth-$2$ ReLU networks under arbitrary distributions without incurring an exponential dependence in {\em both} $n$ and $s$. \pranjal{Raghu: please check this sentence.} 

\begin{proof}
We will prove the claim by designing an {\em improper} learner for the class of $k=1$-sparse ReLU networks. The key idea is that the class of $1$-sparse ReLU networks, i.e., $\cH_{n,s,1}$ is a subclass of size-$s$ decision lists where each node is a halfspace. Recall that a decision list over $n$ Boolean variables $x_1, x_2, \ldots x_n$ is a function that can be expressed as a series of {\em if/else} statements, i.e., {\em if $x_1 > 0$ predict +1, else if $x_2 < 0$ predict -1 and so on}. The size of the list equals the number of conditional statements present in the hypothesis. Analogously, we define a generalized decision list over $n$ Boolean variables which is a hypothesis of the form: {\em if $h_1(x_1, \ldots, x_n) > 0$ predict $g_1(x_1, \ldots, x_n)$, else if $h_2(x_1, \ldots, x_n) < 0$ predict $g_2(x_1, \ldots, x_n)$ and so on}.

Let $\tilde{\cH}_{n,s,1}$ denote the class of size-$s$ generalized decision lists where all of the $g,h$ functions are restricted to be halfspaces. We first notice that the class $\tilde{\cH}_{n,s,1}$ contains the class of $1$-sparse ReLU networks, i.e., $\cH_{n,s,1} \subseteq \tilde{\cH}_{n,s,1}$. To see this observe that any $1$-sparse network of the form $h(x) = \sum_{i=1}^s u_i \sigma(\ang{w_i, x} - b_i)$ can be written as a generalized size-$s$ decision list where $h_i(x) = \sign(\ang{w_i, x} - b_i)$ and $g_i(x) = u_i (\ang{w_i, x} - b_i)$. Here we crucially rely on the assumption that each example activates at most one hidden unit in the network.

We will construct our learning algorithm by the empirical risk minimization principle over the hypothesis class of generalized decision lists. Let $s' = O(s \log m)$ for a sample size $m$ to be chosen later. Given a labeled dataset $S = \{(x_1, y_1), \ldots, (x_m, y_m)\}$ we will output a hypothesis $\tilde{h}(x) \in \tilde{\cH}_{n,s',1}$ such that $h(x_i) = y_i$, for all $(x_i, y_i) \in S$. From standard uniform convergence bounds for squared loss (see Lemma~\ref{lem:pdim-generalization}) we get that with probability at least $1-\delta$ over $S$, a hypothesis consistent with the data will satisfy:
\begin{align}
\label{eq:erm}
    \E_{(x,y) \sim D} \big[ (h(x)-y)^2 \big] &\leq 2R \sqrt{\frac{\Pdim(\tilde{\cH}{n,s',1}) \log(m) + \log(\frac 1 \delta)}{m}},
\end{align}
where $\Pdim(\tilde{\cH}_{n,s',1})$ is the pseudo-dimension \citep{haussler1989generalizing, pollard1984convergence} of the hypothesis class and $R$ is the upper bound on the maximum value of any function in the hypothesis class. Using the bound on the norm of the model weights, we get that $R \leq 2B\sqrt{n}$. 

Next we upper bound the pseudo-dimension of $\tilde{\cH}_{n,s',1}$. In order to do this we prove a general statement (See Lemma~\ref{lem:pdim-general-bound} below) bounding the pseudo-dimension of the class of generalized decision lists that we consider. Using Lemma~\ref{lem:pdim-general-bound} we get that

% Fix $r \in \R$ and define the class $\tilde{\cH}^1_{s'}(r) = \{\sign(h(x) - r): h \in \tilde{\cH}^1_{s'})\}$. It is well known that for any fixed $r$ it holds that $\Pdim(\tilde{\cH}^1_{s'}) \leq \VCdim(\tilde{\cH}^1_{s'}(r))$ \citep{anthony1999neural}. Hence, we will provide a uniform upper bound on the VC dimension of the latter class. Let $\VCdim(\tilde{\cH}^1_{s'}(r)) = d_r$ and consider a set of $d_r$ points that can be shattered. Any labeling of these points can be decomposed into two steps, i) partitioning the points via a decision tree with $s'$ leaves ad each internal node being a halfspace in $\R^n$, and ii) labeling each leaf with a halfspace in $\R^n$. Hence, by the Sauer-Shelah Lemma \citep{shalev2014understanding} the total number of possible labeling of $d_r$ points is at most $d^{n'}_r \cdot d^n_r$ where $n'$ is the VC dimension of the class of decision trees with $s'$ leaves and internal nodes being halfspaces in $\R^n$. This implies that $\VCdim(\tilde{\cH}^1_{s'}(r)) = O((n+n') \log(n+n'))$.

% In order to bound $n'$ we recall that over the Boolean hypercube it is sufficient to consider integer weight halfspaces $\sign(\ang{w, x} - b)$ where each $w_i \in [-M, M]$ and $M = n^{O(n)}$ \citep{hong1988connectionist, muroga1961theory, raghavan1988learning}. Hence, the class of decision trees with $s'$ leaves and internal nodes being halfspaces in $\R^n$ is contained in the class of decision trees with $s'$ leaves over $\ell = (2M)^n$ Boolean variables. From the recent work of \citet{leboeuf2020decision} we get that the VC dimension of this class is bounded by $s' \log(s' \ell)$. Hence we get that
\begin{align}
\label{eq:pdim}
    \Pdim(\tilde{\cH}_{n,s',1}) &= O(n s' \log(s')) \nonumber \\
    &= O(n s \log^2(sm)).
\end{align}

Plugging into Eq.~\ref{eq:erm} we get that
with probability at least $1-\delta$ over $S$, a hypothesis consistent with the data will satisfy:
\begin{align}
\label{eq:erm-2}
    \E_{(x,y) \sim D} \big[ (h(x)-y)^2 \big] &\leq 2R \sqrt{\frac{n s \log(sm) + \log(\frac 1 \delta)}{m}},
\end{align}

Setting the right hand side in the above equation to the desired error $\eps$ gives us the claimed sample complexity bound.

Finally we show the claimed bound on the running time. To find a consistent hypothesis note that since the ground truth network has $s$ hidden units and each example is activated by at most one of them, there must be a unit that activates at least a $1/s$-fraction of the examples. To find such a unit we brute force search over all $(2M)^n$ halfspaces that induce a partition and then check in $\text{poly}(n)$ time (via linear programming) whether the examples on the positive side all lie on a single halfspace. If such a condition holds then we add a new $(h,g)$ pair to the front of the generalized decision list and continue over the remaining dataset. Since each time we remove at least a $1/s$-fraction of the dataset, the process ends in $s \log(m)$ steps and produces in the end a generalized size-$s'$ decision list for $s' = s \log(m)$. Hence, the total runtime equals $O\big((2M)^n \cdot m \cdot \text{poly}(n) \cdot s \log(m) \big) = \tilde{O}(s \cdot m \cdot 2^{\tilde{O}(n)})$.


% decision list of size s, with halfspace decision at each node. Use boosting / iterative elimination.
\end{proof}

\begin{lemma}
    \label{lem:pdim-general-bound}
    Let $\cH$ be a class of Boolean functions from $\cX \mapsto \{-1,+1\}$ and let $\cG$ be the class of real valued functions from $\cX \mapsto \R$. Define a size-$s$ generalized decision list to be a hypothesis of the form: {\em if $h_1(x) > 0$ predict $g_1(x)$, else if $h_2(x) < 0$ predict $g_2(x)$ and so on}, where $s$ is the number of conditional statements, the functions $h_i$ are chosen from $\cH$, and the functions $g_i$ are chosen from $\cG$. Let $\cF_s$ be the class of such size-$s$ generalized decision lists. Then it holds that:
    \begin{align}
        \Pdim(\cF_s) = O\big( (\VCdim(\cH) + \Pdim(\cG)) s \log s \big).
    \end{align}
    \end{lemma}
\begin{proof}
We will use the well known fact that for any real valued function class $\cF_s: \cX \mapsto \R$, $\Pdim(\cF_s) = \VCdim(\tilde{\cF_s})$, where $\tilde{\cF_s}$ is the function class: $\{(x,r) \mapsto \sign(f(x) - r): f \in \cF_s\}$ \citep{anthony1999neural}. Analogously, let $\tilde{\cG}$ be the function class: $\{(x,r) \mapsto \sign(g(x) - r): g \in \cG\}$. Then we have that $\VCdim(\tilde{\cG}) = \Pdim(\cG)$.

Next, note that any function in $\tilde{\cF}_s$ can be written as: $G(h_1(x), h_2(x), \ldots, h_s(x), \sign(g_1(x)-r), \sign(g_2(x)-r), \ldots, \sign(g_s(x)-r))$ where $G$ is a fixed function operating over $2s$ Boolean variables (the fixed function simply outputs coordinate $s+i$ for the first non-negative coordinate $i$ that exits among the first $s$ coordinates). Hence, the function class $\tilde{\cF}_s$ is contained in the function class: $\{G(h_1(x), \ldots, h_{s}(x), \tilde{g}_1(x), \ldots, \tilde{g}_s(x)): h_i \in \cH, \tilde{g}_i \in \tilde{\cG}\}$. Using existing VC dimension bounds on function composition (see Lemma 16 in \citet{attias2022improved}) we get that
\begin{align*}
    \Pdim(\cF_s) &= \VCdim(\tilde{\cF}_s)\\
    &= O \big( (\VCdim(\cH) + \VCdim(\tilde{\cG})) s \log s\big)\\
    &= O\big( (\VCdim(\cH) + \Pdim(\cG)) s \log s \big).
\end{align*}
\end{proof}

% Note: We would have got $(ns)^{O(ns)}$ with assumptions on sparsity.

% \begin{theorem}
% $\cH^1_s$ can be learnt with sample complexity $O(ns)$ and running time $(ns)^{O(s)}$
% \end{theorem}
% \begin{proof}
% enumerating over which node is active for each of the $ns$ examples.
% \end{proof}


\subsection{\boldmath Sparsity \texorpdfstring{$k \ge 1$}{k ge 1}}

The proof of Theorem~\ref{thm:ub-general-1} can be easily adapted to the case of $k$-sparse networks, i.e, $\cH_{n,s,k}$ leading to the following Theorem.

\begin{theorem}
\label{thm:ub-general-k}
$\cH_{n,s,k}$ is $(\epsilon,\delta)$-PAC learnable with sample complexity $m = \tilde{O}\left(\frac{n^2 B^2 s k \log(\frac 1 \delta)}{\epsilon^2} \right)$ and running time $\tilde{O}\left(s \cdot m \cdot 2^{\tilde{O}(nk)}\right)$.
\end{theorem}
\begin{proof}
    See Appendix~\ref{sec:ub-general-k}.
\end{proof}


% \begin{theorem}
% $\cH^k_s$ can be learnt with sample complexity $O(ns)$ and running time $s \cdot 2^{O(nk)}$.
% \end{theorem}
% \begin{proof}
% decision list with intersection-of-$k$-halfspace decision at each node.
% \end{proof}
